Variations of the SIR model for COVID-19 evolution

In this work, we discuss the SIR epidemiological model and different variations of it applied to the propagation of the COVID-19 pandemia; we employ the data of the state of Guanajuato and of Mexico. We present some considerations that can improve the predictions made by those models. We consider a time-dependent infection rate, which we adjust to the data. Starting from a linear regime where the populations are much smaller that the country or state population and the population of susceptible (S) can be approximated in convenient units to S approximately 1, we make fits of the parameters. We also consider the case when the susceptible starts departing from 1, for this case we adjust an effective contagion rate. We also explore the ratio of detected populations and the real ones, obtaining that -for the analyzed case it is of approximately 10%. We estimate the number of deaths by making a fit versus the recovered cases, this fit is in first approximation linear, but other powers can give a good agreement. By predictions to past data, we conclude that adaptations of the SIR model can be of great use in describing pandemia's propagation, specially in limited time periods.

==> Sections/abstract.tex <==
En el presente reporte se analizan datos de infectados, recuperados y fallecidos del estado de Guanajuato empleando un modelo SIR (Suceptibles, Infectados y Recuperados). Se considera una tasa de contagio variable ($\beta$) y se ajusta con datos al {\bf 10.05.21}. Se eval\'ua la taza de recuperaci\'on local ($\gamma$). Se realizan estimados de infectados activos, acumulados, recuperados y fallecidos a una  y tres semanas incluyendo rangos de error.


Hagamos algunas acotaciones:
\begin{itemize}
\item El $4$ de abril del $2020$ es el día 1 a partir del que comienza el conteo que aparece en las \textbf{gráficas de la \ref{fig:Inf7} a la \ref{fig:Dif21} y la \ref{fig:logbeta}}.

\item El \textbf{número de infectados activos} en un día dado se calcula a partir de los datos reportados en el mismo día como el número de infectados acumulados menos los recuperados acumulados y los difuntos acumulados.

\item La \textbf{incertidumbre superior} de cada valor predicho (infectados activos, recuperados acumulados y los difuntos acumulados) es la cota superior para ese valor menos el valor predicho.

\item La \textbf{incertidumbre inferior} es el valor predicho menos la cota inferior.

\item El \textbf{número de infectados acumulados predichos} se calcula como los infectados activos predichos más los recuperados acumulados predichos y los difuntos acumulados predichos.

\item La \textbf{cota superior de la predicción de infectados acumulados} se calcula como los infectados acumulados más la suma de las incertidumbres superiores de infectados activos, recuperados acumulados y difuntos acumulados.

\item La \textbf{cota inferior de la predicción de infectados acumulados} son los infectados acumulados menos la suma de las incertidumbres inferiores de infectados activos, recuperados acumulados y difuntos acumulados.

\item Se referirá el número de difuntos acumulados más recuperados acumulados como los \textbf{inmunes} y esa cifra se denotará como $\tilde{R}$.

\item El número de recuperados fue ajustado linealmente en función de los inmunes (tanto en  la proyecci\'on a 7 y a 21 días). 

\item El número de difuntos fue ajustado linealmente en función de los inmunes (tanto en  la proyecci\'on a 7 y a 21 días). 

\item  En la  \textbf{seccci\'on \ref{sec:pred7}} se reportan las proyecciones a 7 d\'{\i}as.
En la \textbf{sección \ref{sec:pred21}} se reportan las proyecciones a 21 d\'{\i}as.
En la \textbf{ secci\'on \ref{sec:ajustes}} se reporta la tasa de recuperaci\'on $\gamma$, la tasa de 
contagio $\beta$, as\'{\i} como el ajuste de fallecidos contra recuperados.

\end{itemize}  

==> Sections/apendice_vacunados.tex <==
%-------------------------------------------------------------------
\section{Apéndice: Predicciones con el Modelo SIR que considera la vacunación}

El análisis de las secciones pasadas es válido si no se considera el proceso de vacunación. Si se utiliza una modificación en el modelo que considere las personas \textbf{vacunadas} $V$ y una \textbf{velocidad de vacunación} estimada que varía linealmente con el tiempo $\tilde{\beta}(t)$, se producen los siguientes resultados.

Se reportan sólo las gráficas de las predicciones de los infectados activos (gráficas \ref{fig:Inf7_vac} y \ref{fig:Inf21_vac}), pues es donde se puede apreciar una diferencia notable entre las predicciones realizadas con el modelo que considera los vacunados y el modelo que no los toma en cuenta.

\subsection{Predicciones para 7 días}

El número de \textbf{infectados activos} predichos para dentro de 7 días, al 17.05.21, es de $\mathbf{715}$ (con una \textit{cota superior} de $1,017$ y una \textit{cota inferior} de $517$).
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{infectados7dias_vac.png}
    \caption{En los puntos rojos se muestran los casos infectados activos calculados, día a día, desde el 11 de abril del 2021 hasta el 10 de mayo del 2021. En la región azul se encuentran los valores predichos en los siguientes siete días usando un modelo que toma en cuenta la vacunación.}
    \label{fig:Inf7_vac}
\end{figure}

Para el número de \textbf{recuperados acumulados}, dentro de 7 días, al 17.05.21, se tiene una predicción de $\mathbf{120,920}$ (con una \textit{cota superior} de $121,326$ y una \textit{cota inferior} de $120,559$).

%\newpage

Para el número de \textbf{difuntos acumulados}, se tiene una predicción al 17.05.21 de $\mathbf{10,990}$ (con una \textit{cota superior} de $11,068$ y una \textit{cota inferior} de $10,916$).

Para el número de \textbf{infectados acumulados}, se tiene una predicción al 17.05.21 de $\mathbf{132,625}$ (con una \textit{cota superior} de $133,412$ y una \textit{cota inferior} de $131,992$).

%\vfill
%-------------------------------------------------------------------
\subsection{    Predicciones para 21 días.}

La predicción del número de \textbf{infectados activos} para dentro de 21 días, al 31.05.21, es de $\mathbf{404}$ (con una \textit{cota superior} de $751$ y una \textit{cota inferior} de  $238$).
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{infectados21dias_vac.png}
    \caption{En los puntos rojos se muestran los casos infectados activos calculados, día a día, desde el 11 de abril hasta el 10 de mayo del 2021. En la región azul se encuentran los valores predichos para los siguientes veintiún días usando un modelo que toma en cuenta la vacunación.}
    \label{fig:Inf21_vac}
\end{figure}
Para los \textbf{recuperados acumulados}, para dentro de 21 días, al 23.05.21, se tiene una predicción de $\mathbf{121,511}$ (con una \textit{cota superior} de $122,272$ y una \textit{cota inferior} de $120,940$).


Para los \textbf{difuntos acumulados}, se tiene una predicción a 21 días, al 31.05.21, de $\mathbf{11,048}$ (con una \textit{cota superior} de $11,161$ y una \textit{cota inferior} de $10,953$).


Para el número de \textbf{infectados acumulados}, se tiene una predicción al 31.05.21 de $\mathbf{132,964}$ (con una \textit{cota superior} de $134,186$ y una \textit{cota inferior} de $132,131$).

\subsection{La velocidad de vacunación}
En la página de la Secretaría de Salud del Estado de Guanajuato se reportan las vacunas aplicadas. Por la ambigüedad que se encontró en esa definición, se optó por suponer que el número de personas vacunadas es el número de vacunas aplicadas entre dos.

Dado que hay días en los que el número de personas vacunadas no cambia, para el los siguientes cálculos sólo se usaron los datos de los días en los que hubo un cambio en el número (los datos que en la figura \ref{fig:datosvac} aparecen en color naranja).

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{datosvac.png}
    \caption{El número de vacunados acumulados desde el 17 de marzo del 2021 (el día en el que se empezó a reportar el número de vacunas) hasta el 10 de mayo el 2021. Los puntos naranjas son aquellos que se usan para calcular la velocidad de vacunación}
    \label{fig:datosvac}
\end{figure}

La \textbf{velocidad de vacunación} dada en unidades de $[\tilde{\beta}]=$personas$/$d\'{\i}as, se estima con los datos desde el 17 de marzo del 2021 y se ajusta a una función lineal:
\begin{equation*}
    \tilde{\beta} = (-4 \pm 3) t +8,000 \pm 1,000
\end{equation*}                      

Su ajuste en función del día se muestra en la \textbf{figura \ref{fig:velvac}}. Note que esta tasa se construye como el cociente de la cantidad de nuevas personas vacunadas entre el número de días que hay entre cada dato usado (las diferencias en el eje horizontal entre cada punto naranja consecutivo en la figura \ref{fig:datosvac}).

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{betatilde.png}
    \caption{El ajuste lineal entre el valor del la valocidad de vacunación contra el día en el que se obtiene tal valor.}
    \label{fig:velvac}
\end{figure}


==> Sections/conclusiones.tex <==
\section{Conclusiones}
Los datos actualizados de la epidemia en el estado de Guanajuato, analizados con la suposici\'on de un modelo SIR muestran una tendencia a la disminuci\'on de casos activos, sin embargo se proyecta que seguir\'an en el orden de los miles en las pr\'oximas semanas. Esperamos que estas estimaciones sirvan como gu\'{\i}a para el an\'alisis de la situaci\'on actual. Este reporte es un estudio matem\'atico, y sus proyecciones son responsabilidad \'unica de los autores.

\section{Agradecimientos}

 Agradecemos al Programa de Servicio Social de la Universidad de Guanajuato, que nos permiti\'o realizar el proyecto ``Modelación matemática de la epidemia del COVID-19" del cual este reporte es parte, agradecemos a Gabriel Am\'ezquita, Oscar Esaul Cervantes, Juan Carlos God\'{\i}nez e Iv\'an Yebra por su colaboraci\'on en dicho proyecto. Agradecemos a los investigadores: Argelia Bernal, Juan Barranco, Alejandro Cabo, Alma Gonz\'alez, Dami\'an Mayorga, Gustavo Niz y Luis Ure\~na por \'utiles discusiones en esta tem\'atica.  Agradecemos al Laboratorio de Datos de la DCI, UG, el apoyo del proyecto  CIIC 264/2022 UG, y del proyecto CONACyT A1-S-37752.

\newpage
\newpage

==> Sections/tasas.tex <==
\section{La tasa de transmisión ($\beta$), la tasa de recuperación ($\gamma$) y el ajuste de los difuntos.}\label{sec:ajustes}

En las tres gráficas siguientes, los \textbf{puntos azules} son los datos usados, la \textbf{recta roja} es el ajuste de interés en cada caso, la \textbf{región azul} sombreada es el intervalo de confianza del $95$ $\%$ del modelo y las \textbf{curvas grises} en torno al modelo y el intervalo de confianza contienen al intervalo de predicción del $95$ $\%$.

La \textbf{tasa de recuperación efectiva} dada en unidades de $[\gamma_{eff}]=$1/d\'{\i}as, se estima para los últimos 150 días mediante un ajuste lineal como se muestra en la \textbf{figura \ref{fig:gamma}}. Esta tasa es la pendiente de la recta, $\gamma_{eff}$ = ({8.5} $\pm$ {0.3}) $\times$ \num{e-2}.
%Tasa de recuperación efectiva: 0.08517 +/- 0.00282


\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{gamma.png}
    \caption{El ajuste lineal entre los infectados activos al día contra los nuevos casos inmunes. La pendiente de este ajuste es la tasa de recuperación (calculada con la información de los últimos $150$ días).}
    \label{fig:gamma}
\end{figure}

La \textbf{tasa de transmisión} dada en unidades de $[\beta]=$1/(d\'{\i}as$\times$ personas), se estima de los últimos 30 días se ajusta a una exponencial con los siguientes parámetros:
\begin{equation*}
    \beta =  e ^  {(0.0027 \pm 0.0004) t -2.8 \pm 0.1}. 
%Tasa de infección como función del tiempo: exp(0.00289 t + -3.8059) * exp(+/- 0.00038 t +/- 0.14447)
\end{equation*}                      

Su ajuste en función del día se muestra en la \textbf{figura \ref{fig:logbeta}}. Note que esta tasa se construye, día por día, como la suma de $\gamma_{eff}$ con el cociente la cantidad de infecciones nuevas entre las infecciones activas ese día.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{beta.png}
    \caption{El ajuste lineal entre el valor del logaritmo de la tasa de transmisión contra el día en el que se obtiene tal valor. El exponencial de este ajuste es la expresión que se busca de la tasa de transmisión como función del tiempo.}
    \label{fig:logbeta}
\end{figure}

%esto creo falta redactar que no es solo función de los difuntos  aun----------------------------------------
El \textbf{ajuste de los recuperados en función de los inmunes} de los últimos 274 días se muestra en la \textbf{figura \ref{fig:delta}}. Los parámetros se presentan a continuación.
\begin{equation*}
    R = (0.9107 \pm 0.0002) \tilde{R} +800 \pm 20.
\end{equation*}  

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{ajusterecuperados.png}
    \caption{El ajuste lineal entre el número de recuperados acumulados y los inmunes (calculado con la información de los últimos $274$ días).}
    \label{fig:rho}
\end{figure}

El \textbf{ajuste de los difuntos en función de los inmunes} de los últimos 274 días se muestra en la \textbf{figura \ref{fig:delta}}. Los parámetros se presentan a continuación.
%cambie la palabra recuperados por inmunes 
\begin{equation*}
    D = (0.0893 \pm 0.0002) \tilde{R} -800 \pm 20.
    %Ajuste de difuntos en función de inmunes: (0.09042 Rtilde + -904.57) +/- (0.00019 Rtilde +/- 16.7945)
\end{equation*}          



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.58]{ajustedifuntos.png}
    \caption{El ajuste lineal entre el número de difuntos acumulados y los inmunes  (calculado con la información de los últimos $274$ días).}
    \label{fig:delta}
\end{figure}

